Physics at a 100 TeV pp collider: Standard Model processes

This report summarises the properties of Standard Model processes at the 100 TeV pp collider. We document the production rates and typical distributions for a number of benchmark Standard Model processes, and discuss new dynamical phenomena arising at the highest energies available at this collider. We discuss the intrinsic physics interest in the measurement of these Standard Model processes, as well as their role as backgrounds for New Physics searches.

==> 02-pdf/out <==
ewkevln.tex:\includegraphics[width=0.60\textwidth]{figs/sppc_Lumi.pdf}		\label{fig:sppcLumi}
ewkevln.tex:\includegraphics[width=0.60\textwidth]{figs/sppc_LumiRatio.pdf}	\label{fig:sppcLumiRatio}
lumis.tex:\includegraphics[width=0.49\textwidth]{figs/gg_global_100tev_new}
lumis.tex:\includegraphics[width=0.49\textwidth]{figs/qg_global_100tev_new}
lumis.tex:\includegraphics[width=0.49\textwidth]{figs/q2_global_100tev_new}
lumis.tex:\includegraphics[width=0.49\textwidth]{figs/qq_global_100tev_new}
lumis.tex:  \includegraphics[width=0.49\textwidth,page=1]{figs/lumis-nosig-100TeV-PDF4LHC15_nnlo_mc.pdf}\hfill
lumis.tex:  \includegraphics[width=0.49\textwidth,page=2]{figs/lumis-nosig-100TeV-PDF4LHC15_nnlo_mc.pdf}\\
lumis.tex:  \includegraphics[width=0.49\textwidth,page=3]{figs/lumis-nosig-100TeV-PDF4LHC15_nnlo_mc.pdf}\hfill
lumis.tex:  \includegraphics[width=0.49\textwidth,page=4]{figs/lumis-nosig-100TeV-PDF4LHC15_nnlo_mc.pdf}
lumis.tex:\includegraphics[width=0.49\textwidth]{figs/lumirat-summary-nnpdf30}
lumis.tex:\includegraphics[width=0.49\textwidth]{figs/lumirat-summary-pdf4lhc15}
pdfintro.tex:\includegraphics[width=0.93\textwidth]{figs/kinplot}
pdfintro.tex:\includegraphics[width=0.49\textwidth]{figs/xg-smallx-nlo.pdf}
pdfintro.tex:\includegraphics[width=0.49\textwidth]{figs/xu-smallx-nlo.pdf}
pdfintro.tex:\includegraphics[width=0.49\textwidth]{figs/xg-smallx_err.pdf}
pdfintro.tex:\includegraphics[width=0.49\textwidth]{figs/xu-smallx_err.pdf}
pdfintro.tex:\includegraphics[width=0.46\textwidth]{figs/monash-7tev.pdf}
pdfintro.tex:\includegraphics[width=0.49\textwidth]{figs/vincia30-Monash-xMPI100.pdf}
pdfintro.tex:\includegraphics[width=0.49\textwidth]{figs/xu-largex-FCC}
pdfintro.tex:\includegraphics[width=0.49\textwidth]{figs/xd-largex-FCC}
pdfintro.tex:\includegraphics[width=0.49\textwidth]{figs/xg-largex-FCC}
pdfintro.tex:\includegraphics[width=0.49\textwidth]{figs/xubar-largex-FCC}
pdfintro.tex:\includegraphics[width=0.89\textwidth]{figs/psup}
pdfintro.tex:\includegraphics[width=0.49\textwidth]{figs/xg_pdfplot_q2_q2dep-nnlo}
pdfintro.tex:\includegraphics[width=0.49\textwidth]{figs/xu_pdfplot_q2_q2dep-nnlo}
photoninduced.tex:  \includegraphics[scale=0.49]{figs/apfel_nn23qednlo0118_lept_lumi_100tev}
photoninduced.tex:  \includegraphics[scale=0.49]{figs/apfel_nn23qednlo0118_lept_lumi_y_100tev}
photoninduced.tex:  \includegraphics[clip=true, trim=0.cm 3.5cm 0.7cm 1cm, width=0.49\textwidth]{figs/epem_pt10gev_LEP_100tev}
photoninduced.tex:  \includegraphics[clip=true, trim=0.cm 3.5cm 0.7cm 1cm, width=0.49\textwidth]{figs/epem_pt100gev_eta4_LEP_100tev}
photoninduced.tex:  \includegraphics[clip=true, trim=0.cm 3.5cm 0.7cm 1cm, width=0.49\textwidth]{figs/epem_NEW_pt100gev_eta25_LEP_100tev.pdf}
photoninduced.tex:  \includegraphics[clip=true, trim=0.cm 3.5cm 0.7cm 1cm, width=0.49\textwidth]{figs/epem_NEW_pt100gev_eta4_LEP_100tev.pdf}
photoninduced.tex:  \includegraphics[clip=true, trim=0.cm 3.5cm 0.7cm 1cm, width=0.49\textwidth]{figs/ww_noeta_100tev_LEP.pdf}
photoninduced.tex:  \includegraphics[clip=true, trim=0.cm 3.5cm 0.7cm 1cm, width=0.49\textwidth]{figs/ww_eta4_100tev_LEP.pdf}
photoninduced.tex:  \includegraphics[clip=true, trim=0.cm 3.5cm 0.7cm 1cm, width=0.49\textwidth]{figs/ww_NEW_eta25_100tev_LEP}
photoninduced.tex:  \includegraphics[clip=true, trim=0.cm 3.5cm 0.7cm 1cm, width=0.49\textwidth]{figs/ww_NEW_eta4_100tev_LEP}
smallx.tex:  \includegraphics[width=0.495\textwidth,page=1]{figs/gluon_PDF_small-x_comparison_new.pdf}
smallx.tex:  \includegraphics[width=0.495\textwidth,page=2]{figs/gluon_PDF_small-x_comparison_new.pdf}
smallx.tex:  \includegraphics[width=0.49\textwidth,page=3]{figs/gluon_PDF_small-x_comparison_new.pdf}
smallx.tex:  \includegraphics[width=0.49\textwidth,page=4]{figs/gluon_PDF_small-x_comparison_new.pdf}
topparton.tex:\includegraphics[width=16cm]{figs/topPDF}
topparton.tex:  \includegraphics[width=8.2cm]{figs/ttH}
topparton.tex:  \includegraphics[width=7.7cm]{figs/topPDF-dawson}


==> 04-DY/highmass.tex <==
\subsection{High mass $Z$ and $W$ production}
\label{sec:dyan_highmass}
The dilepton mass of DY pairs, at high mass, is shown in
Fig.~\ref{fig:dymass}.
\begin{figure}[h!]
\centering
\includegraphics[width=0.6\textwidth]{figs/dymass}
\caption{Integrated dilepton invariant mass distribution, for one
  lepton family, with $\vert \eta_\ell \vert<2.5$.}
\label{fig:dymass}
\end{figure}



==> 04-DY/out <==
highenergy.tex:\includegraphics[width=0.7\textwidth]{figs/multiWrates}
highenergy.tex:\includegraphics[width=0.9\textwidth]{figs/WinHighEtjet}
highenergy.tex:\includegraphics[width=0.49\textwidth]{figs/Petriello/pTrat_democratic}
highenergy.tex:\includegraphics[width=0.49\textwidth]{figs/Petriello/pTrat_hier}
highenergy.tex:\includegraphics[width=0.49\textwidth]{figs/Petriello/RjW_democratic}
highenergy.tex:\includegraphics[width=0.49\textwidth]{figs/Petriello/RjW_hier}
highmass.tex:\includegraphics[width=0.6\textwidth]{figs/dymass}
inclusive.tex:\includegraphics[width=0.8\textwidth]{figs/wleppt}
inclusive.tex:\includegraphics[height=0.25\textheight]{figs/Ferrera/etaW.pdf}
inclusive.tex:\includegraphics[height=0.25\textheight]{figs/Ferrera/etaZ.pdf}
inclusive.tex:\includegraphics[width=0.6\textwidth]{figs/Ferrera/asy-lep2}
largept.tex:\includegraphics[width=0.45\textwidth]{figs/wpt}
largept.tex:\includegraphics[width=0.46\textwidth]{figs/dymass}
largept.tex:\includegraphics[width=0.49\textwidth]{figs/Petriello/pTW_cum}
largept.tex:\includegraphics[width=0.49\textwidth]{figs/Petriello/pTJ1}
report.tex:% and their figures should all stay in the figs/ subdirectory
smallpt.tex:\includegraphics[height=0.25\textheight]{figs/Ferrera/WqTb}
smallpt.tex:\includegraphics[height=0.25\textheight]{figs/Ferrera/ZqTb}


==> 06-Vqq/_out2_ <==
wbbjMINLO.tex:\includegraphics[width=0.49\textwidth]{figs/WBBJ-NLO-st-Wb-y-050}
wbbjMINLO.tex:\includegraphics[width=0.49\textwidth]{figs/WBBJ-NLO-st-Wb-y-100}
wbbjMINLO.tex:\includegraphics[width=0.49\textwidth]{figs/WBBJ-NLO-st-costhstar-050}
wbbjMINLO.tex:\includegraphics[width=0.49\textwidth]{figs/WBBJ-NLO-st-costhstar-100}


==> 06-Vqq/macros.tex <==
\def\sss{\mathchoice%
{\displaystyle}%
{\scriptstyle}%
{\scriptscriptstyle}%
{\scriptscriptstyle}%
}

\def\GeV{{\ifmmode {\mathrm{ GeV}}\else ${\mathrm{ GeV}}$\fi}}
\def\TeV{{\ifmmode {\mathrm{ TeV}}\else ${\mathrm{ TeV}}$\fi}}
\def\pt{p_{\sss \rm T}}

\def\POWHEG{{\tt POWHEG}}
\def\POWHEGBOX{{\tt POWHEG BOX}}
\def\GOSAM{{\tt GoSam}}
\def\FASTJET{{\tt Fastjet}}
\def\QGRAF{{\tt QGRAF}}
\def\FORM{{\tt FORM}}
\def\GOSAMCONT{{\tt GoSam-contrib}\xspace}
\def\SAMURAI{{\tt SAMURAI}}
\def\GOLEM{{\tt Golem95}}
\def\NINJA{{\tt Ninja}}
\def\SPINNEY{{\tt SPINNEY}}
\def\MG{{\tt MadGraph4}}
\def\MINLO{{MiNLO}}
\def\MiNLO{{MiNLO}}

\def\as{\alpha_{\sss\rm S}}
\def\kt{k_{\sss\rm T}}

\def\Wbb{{\tt Wbb}}
\def\Wbbj{{\tt Wbbj}}



==> 07-VV/VV_Vph.tex <==
\subsection{$VV$ and $V\gamma$ production} 
\label{sec:VV_Vph}
Cover both inclusive and high-mass $VV/V\gamma$-pair production.


==> 07-VV/Vph.tex <==
\subsection{$V\gamma$ production} 
\label{sec:Vph}
Cover both inclusive and high-mass $V\gamma$ production.


==> 09-jets/inclusive.tex <==
\subsection{Inclusive jet and dijet production}
\label{sec:jets_incl}
Figure~\ref{fig:jetpt} shows the integrated rates for the production
of events with at least one jet of transverse momentum $p_T$ larger
than a given threshold. The distribution refers to jets with
pseudorapidity $\eta$ in the range $\vert \eta \vert <
2.5$. Figure~\ref{fig:etaj} shows the probability that events with
jets above certain $p_T$ threshold be contained inside certain $\eta$
ranges. Notice the huge $\eta$ extension, even for jets with $p_T$ in
the TeV range. Assuming integrated luminosities in excess of 1~\iab,
the reach in $p_T$ extends well above 20~TeV. Fully containing and
accurately measuring these jet energies sets important constraints on
the design of calorimeters, e.g. requiring big depth and therefore
large transverse size, with a big impact on the overall dimensions and
weight of the detectors.
\begin{figure}[h!]
\centering
\includegraphics[width=0.5\textwidth]{figs/jetpt}
\caption{Rates of events with one jet of $\vert \eta\vert<2.5$ and
  $p_T>p_{T}^{min}$.} 
\label{fig:jetpt}
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=0.8\textwidth]{figs/etaj}
\caption{Left: acceptance, for jets above various $p_T$ thresholds, to be
  contained within $\vert\eta_j\vert<\eta_{min}$. Right: probability
  to be outside the $\eta_{min}$ acceptance.}
\label{fig:etaj}
\end{figure}
\begin{figure}[h!]
\centering
\includegraphics[width=0.4\textwidth]{figs/mjj100} \hfil
\includegraphics[width=0.4\textwidth]{figs/mjjfrac}
\caption{Left: dijet mass spectra, for different $\eta$
  constraints. Right: partonic composition of dijet final states, as a
function of the dijet mass. }
\label{fig:mjj100}
\end{figure}

These choices become particularly relevant in the context of searches
for high-mass resonances in dijet final states, where the separation
from the continuum background of possibly narrow states requires good
energy resolution.  Figure~\ref{fig:mjj100} shows the rates for QCD
production of final states with a dijet of invariant mass above a
given threshold. We consider two cases: the dijet mass spectrum of all
pairs with jets within $\vert \eta\vert < 5$, and the spectrum limited
to jets produced at large angle in the dijet center of mass ($\vert
\eta_1 - \eta_2 \vert<2$), a configuration which is more typical of
the production and decay of a possible resonance. Notice that,
particularly at the largest masses, the former rates are several
orders of magnitude larger than the latter ones. This is because one
is dominated there by the low-angle scattering. But even for central
production we have rates in excess of 1 event/\iab\ for masses above
50~TeV. The relative partonic composition of central dijet events, as
a function of the dijet mass, is shown in the right plot of
Fig.~\ref{fig:mjj100}. In the region 2~TeV$ \lsim M_{jj} \lsim$20~TeV
the final states are dominated by $qg$ pairs. Above 20~TeV, we find
mostly $qq$ pairs (the $q\bar{q}$ component is greatly suppressed
throughout).



==> 10-Njets/FCC-multijets.tex <==
%\section{Multijets\footnote{Editors: F.Krauss; contributors: alpgen, blackhat, sherpa, aMC@NLO, Robens, Campbell, SB}}
\section{Multijets}
\label{ref:njets}
%\input{global}
\renewcommand{\arraystretch}{1.5}

\subsection{Cross sections}

Representative NLO $K$-factors are presented with democratic cuts on all jets and hierachical cuts
on the leading jet. Additonal analysis parameters were chosen as,
\begin{align*}
  &|\eta_j| < 5 \\
  &{\rm anti-}k_T, R=0.4 \\
  &\text{CT14 (NLO) PDFs}
\end{align*}

\begin{center}
  \begin{tabular}[h]{cccccccc}
    & \multicolumn{7}{c}{$j^n$} \\
    \hhline{~-------}
    & \multicolumn{3}{c}{$p_T^{\rm min}> 50$ GeV} && \multicolumn{3}{c}{$p_T^{\rm min}> 500$ GeV} \\
    \hhline{~---~---}
    $n$ & LO & NLO & K && LO & NLO & K \\
    2 & $289.0^{+8.7}_{-13.6}$ $\mu$b & $-111.0^{+62.5}_{-66.0}$ $\mu$b & $-0.4^{+0.21}_{-0.21}$ && $66.0^{+12.2}_{-9.8}$ nb & $10.4^{+11.3}_{-18.4}$ nb & $0.2^{+0.23}_{-0.26}$ \\
    3 & $28.5^{+7.1}_{-5.4}$ $\mu$b & $15.1^{+3.1}_{-6.8}$ $\mu$b & $0.5^{+0.26}_{-0.30}$ && $1.7^{+0.6}_{-0.4}$ nb & $1.4^{+0.0}_{-0.3}$ nb & $0.8^{+0.27}_{-0.31}$ \\
    4 & $6.9^{+2.9}_{-1.9}$ $\mu$b & $2.2^{+1.3}_{-3.4}$ $\mu$b & $0.3^{+0.40}_{-0.45}$ && $153.2^{+68.3}_{-44.6}$ pb & $132.8^{+0.0}_{-27.9}$ pb & $0.9^{+0.34}_{-0.39}$
  \end{tabular}
\end{center}
We note the NLO result for di-jet production is unstable with democratic jet selection (SB: I don't think this number should be quoted but I include it for now anyway).

Representative NLO $K$-factors with additional cuts on the highest $p_T$ jet,
\begin{center}
  \begin{tabular}[h]{cccccccc}
    & \multicolumn{7}{c}{$j^n$} \\
    \hhline{~-------}
    & \multicolumn{3}{c}{$p_{T,j_1}>100$ GeV $p_T^{\rm min}> 50$ GeV} && \multicolumn{3}{c}{$p_{T,j_1}>1000$ GeV $p_T^{\rm min}> 500$ GeV} \\
    \hhline{~---~---}
    $n$ & LO & NLO & K && LO & NLO & K \\
    2 & $28.8^{+2.7}_{-2.6}$ $\mu$b & $54.1^{+5.9}_{-4.7}$ $\mu$b & $1.9^{+0.03}_{-0.00}$ && $3.4^{+0.7}_{-0.6}$ nb & $5.5^{+0.6}_{-0.5}$ nb & $1.6^{+0.13}_{-0.14}$ \\
    3 & $20.7^{+5.3}_{-4.0}$ $\mu$b & $7.5^{+3.2}_{-6.4}$ $\mu$b & $0.4^{+0.28}_{-0.32}$ && $1.1^{+0.4}_{-0.3}$ nb & $0.8^{+0.1}_{-0.2}$ nb & $0.7^{+0.28}_{-0.32}$ \\
    4 & $5.6^{+2.4}_{-1.6}$ $\mu$b & $1.7^{+1.1}_{-2.8}$ $\mu$b & $0.3^{+0.39}_{-0.45}$ && $106.8^{+47.6}_{-31.1}$ pb & $92.2^{+0.0}_{-20.0}$ pb & $0.9^{+0.34}_{-0.40}$
  \end{tabular}
\end{center}

In both democratic and hierachical $p_T$ cuts we see a decrease in perturbative stability for the low cut around $50 GeV$.

\begin{figure}[t]
  \begin{center}
    \begin{tabular}[h]{cc}
      \includegraphics[width=6cm]{{plots/2j_100TeV_jpt50_R0.4_NLO_jet_pT_1}.pdf} &
      \includegraphics[width=6cm]{{plots/2j_100TeV_jpt50_R0.4_NLO_jet_pT_2}.pdf}
    \end{tabular}
  \end{center}
  \caption{1st and 2nd leading jet $p_T$ for $pp\to2j$ at LO and NLO.}
  \label{fig:2jetpT}
\end{figure}

\begin{figure}[b]
  \begin{center}
    \begin{tabular}[h]{cc}
      \includegraphics[width=6cm]{{plots/3j_100TeV_jpt50_R0.4_NLO_jet_pT_1}.pdf} &
      \includegraphics[width=6cm]{{plots/3j_100TeV_jpt500_R0.4_NLO_jet_pT_1}.pdf} \\
      \includegraphics[width=6cm]{{plots/3j_100TeV_j1pt100_jpt50_R0.4_NLO_jet_pT_1}.pdf} &
      \includegraphics[width=6cm]{{plots/3j_100TeV_j1pt1000_jpt500_R0.4_NLO_jet_pT_1}.pdf} \\
    \end{tabular}
  \end{center}
  \caption{Leading jet $p_T$ for $pp\to3j$ at LO and NLO.}
  \label{fig:3jetpT}
\end{figure}

We also look at the dependence on the K-factor with respect to the anti-$k_T$ jet radius
for $pp\rightarrow 3j$ using a minimum $p_T>250$ GeV,
\begin{center}
  \begin{tabular}[h]{cccc}
    \multicolumn{4}{c}{$j^3 \qquad p_T>250$ GeV} \\
    \hhline{----}
    $R$ & LO & NLO & K \\
    0.2 & $45.6^{+14.1}_{-10.2}$ nb & $22.4^{+5.2}_{-12.9}$ nb & $0.5^{+0.29}_{-0.33}$ \\
    0.3 & $43.4^{+13.5}_{-9.7}$ nb & $27.6^{+3.2}_{-9.7}$ nb & $0.6^{+0.28}_{-0.32}$ \\
    0.4 & $41.8^{+13.0}_{-9.4}$ nb & $30.8^{+1.9}_{-7.5}$ nb & $0.7^{+0.27}_{-0.31}$ \\
    0.5 & $40.5^{+12.6}_{-9.1}$ nb & $33.5^{+0.8}_{-5.8}$ nb & $0.8^{+0.26}_{-0.31}$ \\
    0.6 & $39.3^{+12.3}_{-8.8}$ nb & $35.6^{+0.0}_{-4.3}$ nb & $0.9^{+0.26}_{-0.30}$ \\
    0.7 & $38.2^{+11.9}_{-8.6}$ nb & $36.8^{+0.0}_{-3.2}$ nb & $1.0^{+0.25}_{-0.29}$ \\
  \end{tabular}
\end{center}
as expected even with a relatively high $p_T$ cut perturbative stability is compromised
for $R\lesssim0.3$.

\subsection{Cross sections for $\gamma$+jets}

Representative NLO $K$-factors for photon plus jets final states ae presented with the following
kinematic cuts,
\begin{align*}
  &|\eta_{j/\gamma}| < 8 \\
  &p_{T,\gamma} > p_T^{\rm min} \\
  &p_{T,j} > p_T^{\rm min} \\
  &R_{\gamma,j} > 0.4 \\
  &{\rm anti-}k_T, R=0.4 \\
  &\text{CT14 (NLO) PDFs}
\end{align*}
The Frixione smooth cone isolation was used with $R=0.4$, $\varepsilon=0.1$ and $n=1$. Jets
have been defined using the anti-$k_T$ algorithm using $R=0.4$.

\begin{center}
  \begin{tabular}[h]{cccccccc}
    & \multicolumn{7}{c}{$\gamma\gamma+j^n$} \\
    \hhline{~-------}
    & \multicolumn{3}{c}{$p_T^{\rm min}> 50$ GeV} && \multicolumn{3}{c}{$p_T^{\rm min}> 500$ GeV} \\
    \hhline{~---~---}
    $n$ & LO & NLO & K && LO & NLO & K \\
    1 & $71.6^{+6.5}_{-8.2}$ nb & $115.5^{+5.0}_{-3.1}$ nb & $1.6^{+0.29}_{-0.17}$ && $39.4^{+2.3}_{-2.2}$ pb & $46.9^{+1.4}_{-1.2}$ pb & $1.2^{+0.04}_{-0.03}$ \\
    2 & $24.6^{+2.4}_{-2.2}$ nb & $32.7^{+1.7}_{-1.5}$ nb & $1.3^{+0.07}_{-0.06}$ && $3.9^{+0.8}_{-0.6}$ pb & $4.8^{+0.2}_{-0.3}$ pb & $1.2^{+0.15}_{-0.16}$ \\
    3 & $11.2^{+2.9}_{-2.2}$ nb & $10.1^{+0.0}_{-0.9}$ nb & $0.9^{+0.22}_{-0.25}$ && $654.1^{+206.0}_{-147.9}$ fb & $671.1^{+0.0}_{-32.1}$ fb & $1.0^{+0.24}_{-0.28}$
  \end{tabular}
\end{center}

\subsection{Cross sections for $\gamma\gamma$+jets}

Representative NLO $K$-factors for di-photon plus jets final states are defined with the following kinematic cuts,
\begin{align*}
  &|\eta_{j/\gamma}| < 8 \\
  &p_{T,\gamma} > p_T^{\rm min} \\
  &p_{T,j} > p_T^{\rm min} \\
  &R_{\gamma,j} > 0.4 \\
  &{\rm anti-}k_T, R=0.4 \\
  &\text{CT14 (NLO) PDFs}
\end{align*}
The Frixione smooth cone isolation was used with $R=0.4$, $\varepsilon=0.1$ and $n=1$.

\begin{center}
  \begin{tabular}[h]{cccccccc}
    & \multicolumn{7}{c}{$\gamma\gamma+j^n$} \\
    \hhline{~-------}
    & \multicolumn{3}{c}{$p_T^{\rm min}> 50$ GeV} && \multicolumn{3}{c}{$p_T^{\rm min}> 500$ GeV} \\
    \hhline{~---~---}
    $n$ & LO & NLO & K && LO & NLO & K \\
    0 & $45.7^{+8.6}_{-8.5} $ pb & $100.1^{+3.8}_{-5.2} $ pb & $2.2^{+0.36}_{-0.28} $ && $49.0^{+1.4}_{-1.7} $ fb & $68.7^{+1.4}_{-1.1} $ fb & $1.4^{+0.08}_{-0.06} $ \\
    1 & $27.3^{+0.3}_{-0.6} $ pb & $61.7^{+3.7}_{-3.1} $ pb & $2.3^{+0.19}_{-0.13} $ && $7.3^{+0.7}_{-0.6} $ fb & $12.5^{+1.0}_{-0.9} $ fb & $1.7^{+0.04}_{-0.04} $ \\
    2 & $24.4^{+3.1}_{-2.7} $ pb & $31.6^{+1.3}_{-1.4} $ pb & $1.3^{+0.10}_{-0.10} $ && $2.5^{+0.5}_{-0.4} $ fb & $3.2^{+0.1}_{-0.2} $ fb & $1.3^{+0.15}_{-0.17} $
  \end{tabular}
\end{center}

%\input{scaling}


==> 10-Njets/global.tex <==
\def\SI#1#2{#1\,\rm{#2}}
\def\barn{\rm{b}}
\def\micro{\ensuremath{\mu}}

\def\tableHeaderVPhantom{$\vphantom{\displaystyle{\frac{2^n_A}{2^n_A}}}$}
\def\minptcellNoLine#1{\multicolumn{1}{c}{\SI{#1}{GeV}\tableHeaderVPhantom}}
\def\minptcell#1{\multicolumn{1}{c|}{\SI{#1}{GeV}\tableHeaderVPhantom}}
\def\minptcellDoubleline#1{\multicolumn{1}{c||}{\SI{#1}{GeV}}}
\def\processcell#1{\multicolumn{1}{c|}{#1\tableHeaderVPhantom}}
\def\processcellNoLine#1{\multicolumn{1}{c}{#1\tableHeaderVPhantom}}
%\def\mub#1{#1\,\si{\micro\barn}}
%\def\nb#1{#1\,\si{\nano\barn}}
%\def\pb#1{#1\,\si{\pico\barn}}
%\def\fb#1{#1\,\makebox[\widthof{\si{\micro\barn}}]{\si{\femto\barn}}}
%\def\ab#1{#1\,\si{\atto\barn}}
\def\mub#1{#1\,\micro b\xspace}
\def\nb#1{#1\,nb\xspace}
\def\pb#1{#1\,pb\xspace}
\def\fb#1{#1\,fb\xspace}
\def\ab#1{#1\,ab\xspace}
\def\belowfb{\fb{$< 1$}}
\def\belowab{\ab{$< 1$}}
\def\crossedOutMulticolumn#1{\multicolumn{#1}{c|}{---}}
\def\crossedOutMulticolumnNoLine#1{\multicolumn{#1}{c}{---}}
\renewcommand{\arraystretch}{1.2}
%= equation numeration scheme =====================
%\renewcommand{\theequation}{\arabic{section}.\arabic{equation}}
%\numberwithin{equation}{section}
%= abbreviations ==================================
% == methods ======================================
\def\HqT{H\protect\scalebox{0.8}{qT}\xspace}
\def\POWHEG{P\protect\scalebox{0.8}{OWHEG}\xspace}
\def\MINLO{MiN\protect\scalebox{0.8}{LO}\xspace}
\def\SMCatNLO{S--M\protect\scalebox{0.8}{C}@N\protect\scalebox{0.8}{LO}\xspace}
\def\MCatNLO{M\protect\scalebox{0.8}{C}@N\protect\scalebox{0.8}{LO}\xspace}
\def\MCatLO{M\protect\scalebox{0.8}{C}@L\protect\scalebox{0.8}{O}\xspace}
\def\LOPS{LO$\otimes$PS\xspace}
\def\MEPS{M\scalebox{0.8}{E}P\scalebox{0.8}{S}@LO\xspace}
\def\NLOPS{N\scalebox{0.8}{LO}P\scalebox{0.8}{S}\xspace}
\def\MENLOPS{ME\protect\scalebox{0.8}{NLO}PS\xspace}
\def\MEPSatNLO{M\protect\scalebox{0.8}{E}P\protect\scalebox{0.8}{S}@N\protect\scalebox{0.8{LO}\xspace}} 
\def\CKKW{CKKW\xspace}
\def\UNLOPS{UN\scalebox{0.8}{LO}P\scalebox{0.8}{S}\xspace}
% == other MC codes ===============================
\def\Vegas{V\protect\scalebox{0.8}{EGAS}\xspace}
\def\Herwig{H\protect\scalebox{0.8}{ERWIG}\xspace}
\def\Herwigpp{H\protect\scalebox{0.8}{ERWIG++}\xspace}
\def\Ariadne{A\protect\scalebox{0.8}{RIADNE}\xspace}
\def\Alpgen{A\protect\scalebox{0.8}{LPGEN}\xspace}
\def\Madgraph{M\protect\scalebox{0.8}{AD}G\protect\scalebox{0.8}{RAPH}\xspace}
\def\Madevent{M\protect\scalebox{0.8}{AD}E\protect\scalebox{0.8}{VENT}\xspace}
\def\Blackhat{B\protect\scalebox{0.8}{LACK}H\protect\scalebox{0.8}{AT}\xspace}
\def\Pythia{P\protect\scalebox{0.8}{YTHIA}\xspace}
\def\Jetset{J\protect\scalebox{0.8}{ETSET}\xspace}
\def\Vincia{V\protect\scalebox{0.8}{INCIA}\xspace}
\def\aMCatNLO{aM\protect\scalebox{0.8}{C}@N\protect\scalebox{0.8}{LO}\xspace}
\def\PowhegBox{P\protect\scalebox{0.8}{OWHEG}B\protect\scalebox{0.8}{OX}\xspace}
% == other codes ==================================
\def\FeynRules{F\protect\scalebox{0.8}{EYN}R\protect\scalebox{0.8}{ULES}\xspace}
\def\SpringBases{S\protect\scalebox{0.8}{PRING/}B\protect\scalebox{0.8}{ASES}\xspace}
\def\Professor{P\protect\scalebox{0.8}{ROFESSOR}\xspace}
\def\Rivet{R\protect\scalebox{0.8}{IVET}\xspace}
\def\Jetphox{J\protect\scalebox{0.8}{ET}P\protect\scalebox{0.8}{HOX}\xspace}
\def\Diphox{D\protect\scalebox{0.8}{I}P\protect\scalebox{0.8}{HOX}\xspace}
\def\Resbos{R\protect\scalebox{0.8}{ES}B\protect\scalebox{0.8}{OS}\xspace}
\def\BlackHat{B\protect\scalebox{0.8}{LACK}H\protect\scalebox{0.8}{AT}\xspace}
\def\GoSam{G\protect\scalebox{0.8}{O}S\protect\scalebox{0.8}{AM}\xspace}
\def\Golem{G\protect\scalebox{0.8}{OLEM}95\xspace}
\def\Samurai{S\protect\scalebox{0.8}{AMURAI}\xspace}
\def\MCFM{M\protect\scalebox{0.8}{CFM}\xspace}
\def\OpenLoops{O\protect\scalebox{0.8}{PEN}L\protect\scalebox{0.8}{OOPS}\xspace}
\def\SherpaOpenLoops{S\protect\scalebox{0.8}{HERPA}+O\protect\scalebox{0.8}{PEN}L\protect\scalebox{0.8}{OOPS}\xspace}
\def\Collier{C\protect\scalebox{0.8}{OLLIER}\xspace}
\def\VBFNLO{V\protect\scalebox{0.8}{BF}N\protect\scalebox{0.8}{LO}\xspace}
\def\FastJet{F\protect\scalebox{0.8}{ASTJET}\xspace}
% == own stuff ====================================
\def\Sherpa{S\protect\scalebox{0.8}{HERPA}\xspace}
\def\sherpa{\Sherpa}
\def\Comix{C\protect\scalebox{0.8}{OMIX}\xspace}
\def\Apacic{A\protect\scalebox{0.8}{PACIC++}\xspace}
\def\Amegic{A\protect\scalebox{0.8}{MEGIC++}\xspace}
\def\CSS{C\protect\scalebox{0.8}{SS}\xspace}
\def\Ahadic{A\protect\scalebox{0.8}{HADIC++}\xspace}
\def\Adicic{A\protect\scalebox{0.8}{DICIC++}\xspace}
\def\Hadrons{H\protect\scalebox{0.8}{ADRONS++}\xspace}
\def\Photons{P\protect\scalebox{0.8}{HOTONS++}\xspace}
%= experiments ====================================
\def\LEP{LEP\xspace}
\def\LHC{LHC\xspace}
\def\Tevatron{Tevatron\xspace}
\def\Hera{HERA\xspace}
\def\Aleph{ALEPH\xspace}
\def\Delphi{DELPHI\xspace}
\def\Opal{OPAL\xspace}
\def\DO{D\O\ }
\def\CDF{CDF\xspace}
\def\ATLAS{ATLAS\xspace}
\def\CMS{CMS\xspace}
\def\RunII{Run II\xspace}
%= referencing
\def\SecRef#1{Section~\ref{#1}}
\def\EqRef#1{Equation~(\ref{#1})}
\def\EqRefs#1#2{Equations~(\ref{#1})-~(\ref{#2})}
\def\TabRef#1{Table~\ref{#1}}
\def\FigRef#1{Figure~\ref{#1}}
\def\FigRefs#1#2{Figuress~\ref{#1}-~\ref{#2}}
%= definitions ====================================
%\long\def\symbolfootnote#1#2{\begingroup%
%\def\thefootnote{\fnsymbol{footnote}}\footnote[#1]{#2}\endgroup}
\def\abs#1{\left| #1\right|}
\def\rbr#1{\left( #1\right)}
\def\abr#1{\langle #1\rangle}
\def\cbr#1{\left\{ #1\right\}}
\def\sbr#1{\left[ #1\right]}
\def\im{\imath}
\def\jm{\jmath}
\def\args#1{\{\vec{#1}\}}
\def\argc#1#2{\{\vec{#1}\}_{\rm #2}}
\def\ptmin{p_{\perp,{\rm min}}}
\def\done{{\rm d}}
\def\order{\mathcal{O}}
\def\mc#1{\mathcal{#1}}
\def\mr#1{\mathrm{#1}}
\def\mb#1{\mathbb{#1}}
\def\dst{\displaystyle}
\def\sst{\scriptstyle}
\def\bmap#1#2#3{b_{#1,#2}(#3)}
\def\rmap#1#2#3{r_{\widetilde{#1},\tilde{#2}}(#3)}
\def\sbmap#1#2#3#4{b^{\rm(#1)}_{#2,#3}(#4)}
\def\srmap#1#2#3#4{r^{\rm(#1)}_{\widetilde{#2},\tilde{#3}}(#4)}
\def\nnb{\nonumber}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\def\bi{\begin{itemize}}
\def\ei{\end{itemize}}
\def\hl{\vphantom{$\int_A^B$}}
\def\Hl{\vphantom{$\int\limits_a^b$}}
\def\reserrs#1#2#3{$#1_{-#2}^{+#3}$ pb}

\def\trule{\rule[-1.5mm]{0mm}{6mm}}


%==================================================
\def\todo#1{\textbf{\color{red}#1}}
\def\changed#1{\textbf{\color{blue}#1}}

\makeatletter
\def\thefontsize#1{{#1 The current font size is: \f@size pt\par}}
\makeatother


==> 11-hvq/_tmp_ <==
& $8.8\times 10^3$& $2.0\times 10^3$  & 0.70 & $0.86\times 10^{-4}$ \\ 
& $2.7\times 10^3$& $0.42\times 10^3$ & 0.26e-1 & $0.94\times 10^{-7}$ \\ 
        & 100 TeV/13 TeV               & 3.3 & 4.8 & 27 & 910 \\


& $1.0\times 10^3$& $0.60\times 10^3$ & 0.52 & $0.73\times 10^{-4}$\\
& $0.24\times 10^3$& $0.12\times 10^3$ & 0.19e-1 & $0.71\times 10^{-7}$\\
        & 100 TeV/13 TeV               & 4.2 & 5 & 27 & 1030 \\



& 24.8 & 24.8 & 15.5 & $2.6\times 10^{-2}$\\
0.69     0.69   0.37    2.8e-5

==> 11-hvq/intro.tex <==
Heavy quarks will be copiously produced at a 100 TeV collider.  Charm
and bottom quarks, in particular, have a probability of several
percent to be produced in a $pp$ collisions at 100 TeV. Considering
the large number of concurrent $pp$ interactions in individual bunch
crossings, each bunch crossing will give rise to possibly several
charm or bottom quark pairs. The value of the total production rates
is however poorly known due to both perturbative (missing higher
orders) and parametric uncertainties. Perturbative uncertainties
(which, especially for the total cross sections of charm and bottom,
can be quite significant) are usually estimated by varying the
factorisation and renormalisation scales in the calculation.  These
uncertainties may be somewhat reduced by expressing the calculation in
terms of the heavy quark $\overline{\rm MS}$ mass instead of the pole
one~\cite{Alekhin:2012py}, but they remain quite large in absolute
terms, as shown for example in the case of the total
$\sigma(b\bar{b})$ in Fig.~\ref{fig:bbar-scale-dep}. The results here
were obtained with the ABM11 PDFs~\cite{Alekhin:2012ig}.  The scale
uncertainties corresponding to the vertical bars in
Fig.~\ref{fig:bbar-scale-dep}, for the LO, NLO and NNLO calculations,
are $\sigma(b{\bar b})^{\rm LO} = 1.20~_{-~0.33}^{+~0.56}$~mb,
$\sigma(b{\bar b})^{\rm NLO} = 2.45~_{-~0.56}^{+~0.85}$~mb, and
$\sigma(b{\bar b})^{\rm NNLO} = 3.09~_{-~0.48}^{+~0.42}$~mb.
\begin{figure}[h]
\centering
\includegraphics[width=0.65\textwidth]{figs/bbar-scale-dep}
\caption{
  Sensitivity of the total cross section for $pp \rightarrow b\bar{b}$
  to the factorization scale $\mu_F$ at LO (green, dotted), NLO (blue,
  dashed), NNLO (red, solid) QCD accuracy, with $m_b(m_b)=4.18$ GeV in
  the $\overline{\rm MS}$ mass scheme.  The central line at each order
  denotes the choice $\mu_R = \mu_F$, the upper and the lower line the
  choices $\mu_R = \mu_F/2$ and $\mu_R = 2 \mu_F$ (as indicated
  explicitly for the NNLO results).  The vertical bars give the size
  of the independent variation of $\mu_R$ and $\mu_F$ in the standard
  range $\mu_0/2 \le \mu_R, \mu_F \le 2\mu_0$, respectively, for
  $\mu_0=m_b(m_b)$ and 
  with the restriction that $1/2 \le \mu_R/\mu_F \le 2$.  The arrow
  indicates the scale $\mu_R = \mu_F = 2\mu_0$.  }
\label{fig:bbar-scale-dep}
\end{figure}

Parametric uncertainties are related to the value of the heavy quark
mass (for charm and bottom) and of the parton distribution functions
in the very small-$x$ region that will be probed at 100~TeV. Part of
these uncertainties, including the scale uncertainties, can be reduced
when considering ratios of cross sections at different energies, or
shapes of $y_Q$ distributions, due to intrinsic correlations. This was
exploited for example in analyzing LHC data at various beam energies,
in Refs.~\cite{Zenaiev:2015rfa,Gauld:2015kvh,Cacciari:2015fta}.

On the other hand, and as will be shown in the next sub-section, the
range of $x$ values relevant to inclusive production of charm and
bottom quarks at 100 TeV will extend well below the $10^{-5}$
level. In this region, one can question the reliability of the
fixed-order perturbative calculations, in view of the presence of
large small-$x$ logarithms that may need to be
resummed~\cite{Catani:1990eg,Collins:1991ty,Ball:2001pq}.  On the PDF
side, it is also necessary to rely on assumptions for the PDF
functional behaviour at small $x$ (in presence of potential saturation
effects) and on the very reliability of the standard factorization
framework (see Section~\ref{sec:pdf} for a more detailed discussion).

To highlight the possible problems, we show in Table~\ref{tab:QQbar}
the predictions for charm and bottom total cross sections obtained
with several sets of PDFs.  In the case of the bottom, the spread of
central values is not larger than that due to the scale uncertainties,
although the estimates of PDF uncertainties vary wildly among the
different PDF sets. In the case of the charm, the situation is more
dramatic, particularly if one considers the potentially most accurate
estimates, namely those using NNLO matrix elements and NNLO PDFs. In
this case, the results can be negative, or have a positive/negative
uncertainty spread that largely exceeds the central values, leading to
unphysical results, which are either negative, or which exceed the
total $pp$ cross sections. We notice that, in most of the pathological
cases, the problems are enhanced by the use of NNLO PDFs, while using
NLO PDFs with either the NLO or NNLO matrix elements gives typically
sensible results (although with some residual exceptions). The only
PDF sets that give rather stable results, regardless of the NLO or
NNLO scenario, are the ABM sets and the JR14 set. The very small
systematics obtained with these sets (less than 2\% for JR and less
than 10\% with ABM), however, are likely to be over optimistic,
considering the lack of data in these regions of $x$ and $Q^2$ and
considering the potential uncertainties mentioned above (gluon
saturation effects, resummation, etc).


\begin{table}[h]
\begin{center}
%
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{|l||l|l||l|l|}
\hline
PDF sets
  & $\sigma(c{\bar c})^{\rm NLO}$~[mb]
  & $\sigma(c{\bar c})^{\rm NNLO}$~[mb]
  & $\sigma(b{\bar b})^{\rm NLO}$~[mb]
  & $\sigma(b{\bar b})^{\rm NNLO}$~[mb]
\\[1.5ex]
\hline
ABM11~\cite{Alekhin:2012ig}
  & $ 29.5 \pm 2.7 $
  & $ 36.6 \pm 2.6 $
  & $ 3.57 \pm 0.13 $
  & $ 3.06 \pm 0.11 $
\\[0.5ex]
  &
  & ($ 54.9 \pm 3.8 $)
  &
  & ($ 4.52 \pm 0.18 $)
\\[0.5ex]
\hline
ABM12~\cite{Alekhin:2013nda} \footnote{
  The NNLO PDF sets {\tt abm12lhc\_3\_nnlo} and {\tt abm12lhc\_4\_nnlo}
  together with the corresponding NNLO value of $\alpha_s(M_Z)$ have been used
  in both the NLO and NNLO cross section computations.}
  & $ 17.3 \pm 2.0 $
  & $ 33.2 \pm 2.6 $
  & $ 2.36 \pm 0.10 $
  & $ 2.97 \pm 0.12 $
\\[0.5ex]
\hline
CJ15~\cite{Accardi:2016qay} \footnote{
  The CJ15 PDFs have been determined at NLO accuracy in QCD, 
  with the cross section errors here computed for $T=10$ 
  (i.e., the errors provided by the {\tt CJ15} set are multiplied 10).}
  & $ 18.4~_{-~2.5}^{+~5.3} $
  & $ - $
  & $ 2.67~_{-~0.26}^{+~0.55} $
  & $ - $
\\[0.5ex]
  & 
  & ($ 40.3~_{-~4.6}^{+~10.3} $)
  &
  & ($ 3.42~_{-~0.31}^{+~0.69} $)
\\[0.5ex]
\hline
CT14~\cite{Dulat:2015mca} \footnote{
  The PDF uncertainties quoted by CT14 denote the 90\% c.l. and have been reduced by a factor
  of 1.645 for comparison with the 68\% c.l. uncertainties quoted by other
  groups.}
  & $ 24.7~_{-~3.1}^{+~1315.5}$
  & $ 31.8~_{-~3.0}^{+~624.3}$
  & $ 3.06~_{-~0.25}^{+~5.35}$
  & $ 3.12~_{-~0.21}^{+~3.39}$
\\[0.5ex]
  &
  & ($ 47.9~_{-~5.2}^{+~1981.2}$)
  &
  & ($ 3.91~_{-~0.30}^{+~6.91}$)
\\[0.5ex]
\hline
HERAPDF2.0~\cite{Abramowicz:2015mha} \footnote{
  The model uncertainties of the {\tt HERAPDF20\_NNLO\_VAR} set are not included in the 
  uncertainty estimates.}
  & $ 19.0~_{-~4.4}^{+~3.8}$
  & $  3.2~_{-~18.2}^{+~10.1}$
  & $ 3.14~_{-~0.13}^{+~0.10}$
  & $ 2.70~_{-~0.22}^{+~0.21}$
\\[0.5ex]
  &
  & ($ 41.5~_{-~5.9}^{+~5.2}$) 
  &
  & ($ 4.01~_{-~0.16}^{+~0.13}$)
\\[0.5ex]
\hline
JR14 (dyn)~\cite{Jimenez-Delgado:2014twa} 
  & $ 33.6 \pm 0.5 $
  & $ 32.7 \pm 0.5 $
  & $ 3.17 \pm 0.04 $
  & $ 3.08 \pm 0.04 $
\\[0.5ex]
&
& ($ 58.1 \pm 1.0 $) 
&
& ($ 3.98 \pm 0.06 $)
\\[0.5ex]
\hline
MMHT14~\cite{Harland-Lang:2014zoa} \footnote{
  The cross section prediction for $\sigma(c{\bar c})^{\rm NNLO}$ with the
  MMHT14 PDF set at NNLO does not yield a positive value.}
  & $ 140.0~_{-~104.2}^{+~187.0}$
  & $ - $
  & $ 4.11 ~_{-~0.90}^{+~1.39}$
  & $ 2.37 ~_{-~0.90}^{+~0.98}$
\\[0.5ex]
&
& ($ 213.9~_{-~149.4}^{+~271.9}$)
&
& ($ 5.28 ~_{-~1.14}^{+~1.77}$)
\\[0.5ex]
\hline
NNPDF3.0~\cite{Ball:2014uwa}
  & $  40.5 \pm 62.2 $
  & $ 190.3 \pm 547.7 $
  & $  2.99 \pm 0.99 $
  & $  4.46 \pm 4.87 $
\\[0.5ex]
&
& ($ 67.9 \pm 84.3 $)
&
& ($ 3.82 \pm 1.23 $)
\\[0.5ex]
\hline
\end{tabular}
%
  \caption{\small 
    \label{tab:QQbar}
    The inclusive cross sections for charm- and bottom-quark pair
    production at NNLO in QCD at $\sqrt{s}=100$~TeV for
    $\overline{\mathrm{MS}}\, $ masses $m_c(m_c)=1.275$~GeV and
    $m_b(m_b)=4.18$~GeV at the nominal scales $\mu_r=\mu_f=2m_q(m_q)$
    for $q=c,b$ with the PDF (and, if available, also $\alpha_s$)
    uncertainties.  The numbers in parenthesis for the cross sections
    $\sigma(q{\bar q})^{\rm NNLO}$ have been obtained with NLO PDF
    sets.  }
\end{center}
\end{table}


The bottom line is that, while currently the extrapolation of charm
cross sections to 100 TeV is not robust theoretically, charm
production provides a rich terrain to improve our knowledge of PDFs
and small-$x$ dynamics.

The uncertainties are reduced if one considers central production or
large $p_T$, which strongly bound the relevant $x$ range.  Table
\ref{sect11:tab1} shows the rates for central production, $|y|<2.5$,
and various transverse momentum cuts for charm, bottom and top
quarks. The ratios with respect to the production at the LHC (13 TeV)
are also given. As expected, large $p_T$ production in particular gets
a large boost from 13 to 100 TeV, being larger by a factor of 30-40 or
so than at the LHC for a $p_T$ cut of 100 GeV. If the $p_T$ cut is
pushed to 1 TeV, central heavy quark production at the 100~TeV is
about a factor of one thousand larger than at the LHC.  Top production
is special in that, as expected, going from the LHC to 100~TeV the
rate increases considerably also at moderate transverse momentum ($p_T
\sim 0$), by a factor of 40 or so, whereas charm and bottom production
only increase by a factor of 3-5.

\begin{table}[h]
\begin{center}
\begin{tabular}{c|c|c|c|c|c}
\hline
&& $p_T > 0$ & $p_T > 5$ GeV & $p_T > 100$ GeV & $p_T > 1000$ GeV  \\
\hline
\multirow{2}{*}{Charm}  & $\sigma(|y| < 2.5)$ [$\mu$b] & $7.8\times
10^3$& $1.7\times 10^3$ & 0.52 & $0.62\times 10^{-4}$ \\
                        & 100 TeV/13 TeV               & 3.1 & 4.6 & 27 & 890 \\
			\hline
\multirow{2}{*}{Bottom} & $\sigma(|y| < 2.5)$ [$\mu$b] & $1.0\times 10^3$& $0.56\times 10^3$ &0.46 & $0.63\times 10^{-4}$\\
                        & 100 TeV/13 TeV               & 4.2 & 5 & 27 & 1020 \\
			\hline
\multirow{2}{*}{Top}    & $\sigma(|y| < 2.5)$ [nb] & 24.8 & 24.8 & 15.6 & $2.6\times 10^{-2}$\\
                        & 100 TeV/13 TeV               & 37 & 37 & 42 & 920 \\
\hline
\end{tabular}
\caption{\label{sect11:tab1} Central ($|y|<2.5$) heavy quark
  production at FCC 100 TeV, calculated to next-to-leading
  order~\cite{Nason:1987xz} with the NNPDF30~\cite{Ball:2014uwa} PDF
  set. Masses have been set to 1.5 GeV for charm, 4.75 GeV for bottom
  and 173 GeV for top.}
\end{center}
\end{table}

%MLM table:
%\begin{table}[h]
%\begin{center}
%\begin{tabular}{c|c|c|c|c|c}
%\hline
%&& $p_T > 0$ & $p_T > 5$ GeV & $p_T > 100$ GeV & $p_T > 1000$ GeV  \\
%\hline
%\multirow{2}{*}{Charm} & $\sigma(|y| < 2.5)$ [$\mu$b]
%& $8.8\times 10^3$& $1.8\times 10^3$ & 0.53 & $0.62\times 10^{-4}$ \\ 
%        & 100 TeV/13 TeV               & 3.2 & 4.7 & 27 & 890 \\
%			\hline
%\multirow{2}{*}{Bottom} & $\sigma(|y| < 2.5)$ [$\mu$b]
%& $1.1\times 10^3$& $0.59\times 10^3$ & 0.46 & $0.63\times 10^{-4}$\\
%        & 100 TeV/13 TeV               & 4.3 & 5.2 & 27 & 1030 \\
%			\hline
%\multirow{2}{*}{Top}    & $\sigma(|y| < 2.5)$ [nb]
%& 24.8 & 24.8 & 15.5 & $2.6\times 10^{-2}$\\
%        & 100 TeV/13 TeV               & 36 & 36 & 42 & 930 \\
%\hline
%\end{tabular}
%\caption{\label{sect11:tab1} Central ($|y|<2.5$) heavy quark
%  production at FCC 100 TeV, calculated to next-to-leading
%  order~\cite{Nason:1987xz} with the NNPDF30~\cite{Ball:2014uwa} PDF
%  set. Masses have been set to 1.5 GeV for charm, 4.75 GeV for bottom
%  and 173 GeV for top. $\mu_R^2=\mu_F^2=m_Q^2+p_T^2$.}
%\end{center}
%\end{table}


In the rest of this Section we will consider in more detail production
rates and kinematical distributions for bottom and top quark in
proton-proton collisions at a centre of mass energy of 100 TeV.



==> 11-hvq/tmp <==
& $8.8\times 10^3$& $2.0\times 10^3$  & 0.70 & $0.86\times 10^{-4}$ \\ 
& $2.7\times 10^3$& $0.42\times 10^3$ & 0.26e-1 & $0.94\times 10^{-7}$ \\ 
        & 100 TeV/13 TeV               & 3.3 & 4.8 & 27 & 910 \\


& $1.0\times 10^3$& $0.60\times 10^3$ & 0.52 & $0.73\times 10^{-4}$\\
& $0.24\times 10^3$& $0.12\times 10^3$ & 0.19e-1 & $0.71\times 10^{-7}$\\
        & 100 TeV/13 TeV               & 4.2 & 3.8 & 27 & 1030 \\


==> 12-top/out2 <==
davide.tex:\includegraphics[scale=0.65]{figs/Fig_ttbgamma_decay.pdf}
report.tex:% and their figures should all stay in the figs/ subdirectory
tprop.tex:\includegraphics[scale=0.3]{./figs/chromo_fig4.pdf}
tprop.tex:\includegraphics[scale=0.3]{./figs/chromo_fig5.pdf}
tprop.tex:\includegraphics[scale=0.4]{./figs/LHC_C1_3000.pdf}\hspace{10mm}
tprop.tex:\includegraphics[scale=0.4]{./figs/LHC_C2_3000.pdf}\\[5mm]
tprop.tex:\includegraphics[scale=0.4]{./figs/FCC_C1.pdf}\hspace{8mm}
tprop.tex:\includegraphics[scale=0.4]{./figs/FCC_C2.pdf}
tprop.tex:\includegraphics[height=5cm]{./figs/Zt-13} &
tprop.tex:\includegraphics[height=5cm]{./figs/Zt-100} \\
tprop.tex:\includegraphics[height=5cm]{./figs/At-13} &
tprop.tex:\includegraphics[height=5cm]{./figs/At-100}


==> 12-top/ttpho.tex <==
\subsection{$t\bar{t}\gamma$ production}
\label{sec:ttpho}


==> 12-top/ttw.tex <==
\subsection{$t\bar{t}W$ production}
\label{sec:ttw}
Includes anomalous couplings, etc


==> 12-top/ttz.tex <==
\subsection{$t\bar{t}Z$ production}
\label{sec:ttz}
Includes anomalous couplings, etc


==> 14-loop/intro.tex <==
Loop-induced processes are defined as processes that do not receive
any contribution from tree-level Feynman-diagrams.  Such processes are
especially relevant in the case of the SM Higgs boson, which does not
couple directly to massless partons and is therefore produced
predominantly via gluon fusion, through a loop of heavy quarks.  In
the case of single Higgs production, the effective theory obtained by
integrating out the top quark running in the loop provides a good
approximation and the corresponding cross-section for $g g\rightarrow
H$ has been computed up to $N^3$LO
in~\cite{Anastasiou:2015vya}. Corrections due to finite bottom and top
quark mass effects have been computed at lower orders
in~\cite{Mueller:2015lrx,Banfi:2013eda} and give rise to the largest
theoretical error at N3LO (see the Higgs Chapter of this Report for a
more detailed discussion).

Because of its relevance for the measurement of the trilinear Higgs
self-interaction, the case of Higgs pair production has also been
extensively studied and the $NNLO$ inclusive cross-section in the
heavy top-quark limit was presented in~\cite{deFlorian:2013jea}, later
supplemented by the resummation of the next-to-next-to-leading
logarithms in the threshold expansion
$\frac{m^2_{HH}}{\hat{s}}\rightarrow 1$, where $m_{HH}$ the invariant
mass of the Higgs pair and $\hat{s}$ the partonic center-of-mass
energy. Corrections from top-quark mass effects are expected to be
large in Higgs pair production, but their exact analytic expression
are still unknown at NLO accuracy. However, the impact of these
corrections on the inclusive cross-section has recently been computed
in~\cite{Borowka:2016ehy}, using {\sc\small
  SecDec}~\cite{Borowka:2015mxa} for evaluating the analytically
unknown two-loop master integrals.  Also, partial results including
the exact top quark mass dependence everywhere except in the double
virtual contribution are presented in~\cite{Frederix:2014hta}, while
the work of~\cite{Grigo:2013rya,Grigo:2015dia} presents the complete
top-quark mass effects in an expansion up to terms of
$\mathcal{O}(\frac{1}{m_t^8})$.


For many final states, the gluon-initiated loop-induced process $g g
\rightarrow \{X\}$ is actually a NNLO correction to the corresponding
process $p p \rightarrow \{X\}$ with initial state quarks. However,
because of the large gluon luminosity, the $gg$ contribution is often
non-negligible.  For example, as reported in~\cite{Cascioli:2014yka},
it amounts to $\sim 60$\% of the total NNLO correction to $p p
\rightarrow Z Z$.  Furthermore, the difference in the quark and gluon
PDFs and in the production topologies often cause the kinematic
dependence of the gluon-fusion contribution to be very different from
the corresponding tree-level one, so that a global rescaling of the LO
distributions is not applicable. This fact is illustrated in
Fig.~\ref{fig:TreeVsLoop}, showing the differential distribution of
the transverse momenta of bosons in the processes $p p \rightarrow W^+
W^-$, $p p \rightarrow Z Z$ and $p p \rightarrow Z H$. The difference
in shape is particularly manifest for the $p p \rightarrow Z H$
process because the tree-level contribution, in this case, is
exclusively an $s$-channel process.
\begin{figure}[h!]
	\centering
	\includegraphics[trim=10 0 40 20,clip,scale=0.40]{figs/wpwm.pdf}
	\includegraphics[trim=10 0 40 20,clip,scale=0.40]{figs/zz.pdf}
	\includegraphics[trim=10 0 40 20,clip,scale=0.40]{figs/zh.pdf}
	\caption{\label{fig:TreeVsLoop} Comparison of the transverse momentum of bosons produced in pair at tree-level and via gluon-fusion.}
\end{figure}

With the extensive availability of one-loop matrix elements providers
\cite{Hirschi:2011pa,Hahn:2000kx,Hahn:1998yk,Cascioli:2011va,Cullen:2011ac},
the computation of the loop-induced matrix-element is now
straightforward.  However, the automation of the tools to compute
inclusive cross-sections and generate events is only done in a fully
automatic (and public) way in the {\sc\small MadGraph5\_aMC@NLO}
Monte-Carlo framework, for arbitrary loop-induced processes at
LO~\cite{Hirschi:2015iia}.  Except when otherwise stated, all results
of this section are obtained using this framework.


==> 16-EW/ttv-tthew.tex <==
\subsection{$t \bar t V$ and $t \bar t H$ production}\label{sec:ttv-tth}
%===============================================================================

